Queuing Theoretic Analysis of Power-performance Tradeoff in Power-efficient Computing

In this paper we study the power-performance relationship of power-efficient computing from a queuing theoretic perspective. We investigate the interplay of several system operations including processing speed, system on/off decisions, and server farm size. We identify that there are oftentimes "sweet spots" in power-efficient operations: there exist optimal combinations of processing speed and system settings that maximize power efficiency. For the single server case, a widely deployed threshold mechanism is studied. We show that there exist optimal processing speed and threshold value pairs that minimize the power consumption. This holds for the threshold mechanism with job batching. For the multi-server case, it is shown that there exist best processing speed and server farm size combinations.

==> Simulation.tex <==
\section{Simulation Results}
\label{sec.simulationresults}
In this section we present our simulation results. We choose the simulation parameters from real data traces in many literatures (see \cite{MeisnerGold} and the references therein). Among those parameters we present the simulations that offers the best graphical presentation. 

\subsection{Threshold algorithm}
We consider a computing facility with $P_0 = 150$, $\mu = 1$ and $\lambda = 0.1$ which models low utilization scenario. If the wake up cost is negligible, i.e., $\tau_s = 0$, then from previous analysis we have $\tau_c = 0$ and the mean response time and power consumption reduce to (\ref{eq.R_Ts0}) and (\ref{eq.P_Ts0}) respectively. Figure.~\ref{fig.Ts0Tc0} illustrates the power delay tradeoff for various $C$ when $\tau_s = \tau_c = 0$. 
\begin{figure}[t]
\centering
\includegraphics[scale=0.5]{figures/Ts0Tc0.eps}
\caption{Power delay tradeoff with $\tau_s = \tau_c = 0$. Note that there is an optimal frequency that minimizes the power consumption.}
\label{fig.Ts0Tc0}
\end{figure}
Notice that there is an optimal frequency scaling $f^*$ that minimizes the power consumption. The results suggest that running jobs at large delay (using low frequency) may actually consume more power to run. 

In a more generalized scenario where $\tau_s \neq 0$, Figure~\ref{fig.Tsnot0} validates our argument that there is an optimal $(\tau_c, f)$ pair that jointly minimizes the power consumption given a target mean response time (c.f.~(\ref{eq.P_Tsnot0})). We set $P_0 = 150$, $C = 70$, $\lambda = 0.1$, $\mu = 1$ and $\tau_s = 10$.
\begin{figure}[t]
\centering
\includegraphics[scale=0.5]{figures/Tsnot0.eps}
\caption{Power delay tradeoff with $\tau_s = 10$. Different target delay corresponds to different $\tau_c$ and $f$ pair.}
\label{fig.Tsnot0}
\end{figure}
Notice that for a given mean response time $R'$, there is an optimal $\tau_c$ and an associated frequency scaling $f$ that minimize the power consumption. Note also that for the mean response time achieved by the race-to-halt mechanism ($\tau_c = 0$, $f = 1$), we can pick another $(\tau_c, f)$ pair that yields smaller power consumption. 


\subsection{Threshold algorithm with job batching}
We simulate the mean response time (\ref{eq.threshold_batching_RtoH_R}) and power (\ref{eq.threshold_batching_RtoH_P}) for the threshold algorithm with job batching. We set $P_0 = 150$, $C = 70$, $\lambda = 0.1$, $\mu = 1$, $\tau_s = 10$ and $\tau_c = 0$. The frequency scaling $f$ and batching period $\tau_w$ are kept as variables. The power and delay tradeoff is shown in Figure~\ref{fig.BatchTc0}.
\begin{figure}[t]
\centering
\includegraphics[scale=0.5]{figures/BatchTc0.eps}
\caption{Power delay tradeoff with job batching, $\tau_s = 10$ and $\tau_c = 0$. Different target delay corresponds to different $\tau_w$ and $f$ pair. Note that the curve with $\tau_w = 0$ is the same as the one with $\tau_c = 0$ in Figure~\ref{fig.Tsnot0}.}
\label{fig.BatchTc0}
\end{figure}
Notice that for some mean response time achieved by the race-to-halt mechanism, we can pick another $(\tau_c, f)$ pair that yields smaller power consumption. The intuition is that to save power, one typically prefers smaller $f$ over $f = 1$. However to maintain the same delay performance one needs to compensate the increase in delay caused by smaller $f$ by picking a smaller $\tau_w$. Meanwhile, one should not decrease $f$ too much either as doing so the platform power will soon be the dominating factor. We also note that the power delay tradeoff is monotonic for race-to-halt scheme: increasing $\tau_w$ always incurs larger delay and lower power consumption.  

\subsection{Flow splitting}
We simulate the mean response time and power consumption for multi-server flow splitting case. The case for job splitting shares the same spirit. To illustration purposes we set $P_0 = 150$, $C = 10$, $\lambda = 0.7$ and $\mu = 1$. The frequency scaling $f$ and the number of servers $n$ are kept as variables. Simulation results are shown in Figure~\ref{fig.flowsplit}.
\begin{figure}[t]
\centering
\includegraphics[scale=0.48]{figures/flowsplit.eps}
\caption{Power delay tradeoff with flow splitting.}
\label{fig.flowsplit}
\end{figure}
We note that given a target delay objective, there is an optimal plant size and operating frequency pair that jointly minimizes the power consumption. Generally speaking, in one extreme case where jobs can tolerate long delay, the system should run slowly with small amount of servers (c.f.~(\ref{eq.optimal_flowsplit_freq}) and (\ref{eq.optimal_flowsplit_n})). In another extreme case where jobs demand fast response, the system should run faster with many severs powered on. 

==> styles/def.tex <==

\usepackage{epsfig}
\usepackage{amssymb} 
\usepackage{amsthm}
\usepackage[tbtags]{amsmath} 
\usepackage{graphics,eepic,epic}
\usepackage{latexsym}
\usepackage{euscript}
\usepackage{subfigure}
\usepackage{graphics,eepic,epic,psfrag}



% \input{styles/gww_defs} %%%%%%%%%% Use these style files next time
% \input{styles/gww_chars}
% \input{styles/defs}


\newcommand{\cX}{\mathcal{X}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\sX}{\mathsf{X}}
\newcommand{\sn}{\mathsf{n}}
\newcommand{\sh}{\mathsf{h}}
\newcommand{\fRe}{\mathfrak{Re}}
\newcommand{\fIm}{\mathfrak{Im}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\sRSSI}{\mathsf{RSSI}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cCN}{\mathcal{CN}}
\newcommand{\sU}{\mathsf{U}}
\newcommand{\sY}{\mathsf{Y}}
\newcommand{\sy}{\mathsf{y}}
\newcommand{\sx}{\mathsf{x}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\sH}{\mathsf{H}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\sr}{\mathsf{r}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\sA}{\mathsf{A}}
\newcommand{\sB}{\mathsf{B}}
\newcommand{\vars}{\mathsf{s}}
\newcommand{\sw}{\mathsf{w}}

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}

\usepackage{cite}

